Solvability of the Dirichlet problem using a weaker Carleson condition in the upper half plane

We study an elliptic operator $L:=\mathrm{div}(A\nabla \cdot)$ on the upper half plane $\mathbb{R}^2_+$. There are several conditions on the behavior of the matrix $A$ in the transversal $t$-direction that yield $\omega\in A_\infty(\sigma)$. These include the $t$-independence condition, a mixed $L^1-L^\infty$ condition on $\partial_t A$, and Dini-type conditions. We introduce an $L^1$ Carleson condition on $\partial_t A(x,t)$ that extends the class of elliptic operators for which we have $\omega\in A_\infty(\sigma)$, i.e. solvability of the $L^p$ Dirichlet problem for some $1<p<\infty$.

==> Discoard.tex <==
%Proof of Lemma 8.2 partial derivative ogf w_s^2, \nabla w_s^2
    
    For \ref{lemma:Linenablaw_s^2spatialL^2Bound} we use similar tools. Analogously we get
    \begin{align*}
        &\Vert\eta^2\tau \nabla e^{-(\eta^2s^2-\tau^2)L^s}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2\tau^2,s))\Vert_{L^2(\mathbb{R}^n)}
        \\
        &\qquad=\Vert\eta^2 \nabla \partial_\tau e^{-(\eta^2s^2-\tau^2)L^s}(L^s)^{-1}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2\tau^2,s))\Vert_{L^2(\mathbb{R}^n)}
        \\
        &\qquad\lesssim \frac{1}{\sqrt{\eta^2s^2-\tau^2}}\Vert\eta^2\nabla(L^s)^{-1}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2\tau^2,s))\Vert_{L^2(\mathbb{R}^n)}
            \\
        &\qquad\lesssim \frac{1}{\sqrt{\eta^2s^2-\tau^2}}\Vert\eta^2\partial_s A(\cdot,s)\nabla w(x,\eta^2\tau^2,s))\Vert_{L^2(\mathbb{R}^n)}
            \\
        &\qquad\lesssim \frac{\eta^2}{\sqrt{\eta^2s^2-\tau^2}}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}\Vert\nabla w(x,\eta^2\tau^2,s))\Vert_{L^2(\mathbb{R}^n)}
            \\
        &\qquad\lesssim \frac{\eta^2}{\sqrt{\eta^2s^2-\tau^2}}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}\Vert\nabla \phi^s\Vert_{L^2(\mathbb{R}^n)}
            \\
        &\qquad\lesssim \frac{\eta^2}{\sqrt{\eta^2s^2-\tau^2}}\Vert\partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}|\Delta|^{1/2}.
    \end{align*}

    Again, applying Minkowski inequality gives
    \begin{align*}
        \Vert \nabla w_s^{(2)}(\cdot,s)\Vert_{L^2(\mathbb{R}^n)}&=\int_0^{s} \Vert\eta^2\tau \nabla e^{-(\eta^2s^2-\tau^2)L^s}\Div(\partial_s A(\cdot,s)\nabla w(x,\eta^2\tau^2,s))\Vert_{L^2(\mathbb{R}^n)} d\tau
        \\
        &\lesssim \int_0^{s}\frac{\eta^2}{\sqrt{\eta^2s^2-\tau^2}}\Vert \partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}|\Delta|^{1/2}d\tau
        \\
        &\lesssim \Vert \partial_s A(\cdot,s)\Vert_{L^\infty(\mathbb{R}^n)}|\Delta|^{1/2}.
    \end{align*}



==> HodgeDecomposition.tex <==
\section{Hodge decomposition}

For each \(s>0\) we can find a Hodge decomposition consisting of \(\phi^s\in W_0^{1,2}(3\Delta)\) and \( h^s\in L^2(\Omega)\), where \(h^s\) is divergence free and
\[c(x,s)\chi_{3\Delta}(x)=\AP(x,s)\nabla\phi^s(x)+h^s(x).\]
From Proposition 4 of \cite{hofmann_dirichlet_2022} we know 
\begin{align}\fint_{3\Delta}|\nabla\phi^s|^2 dx\leq C(n,\lambda_0,\Lambda_0).\label{equation:L2ofnablaphiBounded}\end{align}
Furthermore we can observe that for the test function \(v\in C_0^\infty(3\Delta)\)
\[\int_{3\Delta}\AP(x,s)\nabla\phi^s(x)\cdot\nabla v(x) dx=\int_{3\Delta}c(x,s)\cdot\nabla v(x)\]
implies through differentiating both sides with respect to s
\begin{align*}\int_{3\Delta} \AP(x,s)\nabla\partial_s\phi^s(x)\cdot\nabla v(x) dx&= - \int_{3\Delta}\partial_s \AP(x,s)\nabla\phi^s(x)\cdot\nabla v(x) dx 
\\
&\qquad + \int_{3\Delta}\partial_s c(x,s)\cdot\nabla v(x).\end{align*}
Inserting \(v=\partial_s\phi^s\) leads to

\begin{align*}
\lambda_0\Vert \nabla\partial_s\phi^s\Vert_{L^2(3\Delta)}^2&\leq \Big|\int_{3\Delta} \AP(x,s)\nabla\partial_s\phi^s\cdot\nabla\partial_s\phi^s dx\Big|
\\
&\leq\Big|\int_{3\Delta}\partial_s \AP(x,s)\nabla\phi^s(x)\nabla\partial_s\phi^s(x) dx\Big|
\\
&\qquad+ \Big|\int_{3\Delta}\partial_s c(x,s)\cdot\nabla\partial_s\phi^s(x) dx\Big|
\\
&\lesssim\Vert \partial_s\AP\nabla\phi^s\Vert_{L^2(3\Delta)}\Vert \nabla\partial_s\phi^s\Vert_{L^2(3\Delta)} 
\\
&\qquad + \Vert\partial_s c(\cdot,s)\Vert_{L^2(3\Delta)}\Vert\nabla\partial_s\phi^s\Vert_{L^2(3\Delta)},
\end{align*}

and hence 

\begin{align}
\Vert \nabla\partial_s\phi^s\Vert_{L^2(3\Delta)}&\lesssim \Vert \partial_s\AP\nabla\phi^s\Vert_{L^2(3\Delta)} + \Vert\partial_s c(\cdot,s)\Vert_{L^2(3\Delta)}.\label{equation:L2ofpartial_snablaphiBounded}
\end{align}

Analogously we can find a Hodge decompositon of \(b\), i.e. a family of functions \(\tilde{\phi}^s\) such that \(b\chi_{3\Delta}=\AP\nabla\tilde{\phi}^s+\tilde{h}^s\). All the results about \(\phi^s\) hold analogously for \(\tilde{\phi}^s\).

Let us also note that the condition (???) guarantees that we can extend \(A(x,s)\) continuously in \(s=0\) by an elliptic matrix \(A(x,0)\), which has the same ellipticity constant and emits a Hodge decomposition with \(\phi^0\) in the same manner.

\section{Approximation function \(\rho\) and difference function \(\theta\)}

Let \(\eta>0\) be a parameter to be determined later. We define 
\[w(x,t,s):=e^{-tL^s}\phi^s(x)\]
as the solution to the ("t-independent") heat equation
\[\begin{cases} \partial_t w(x,t,s)-L^s w(x,t,s)=0 &,(x,t)\in \Omega \\ w(x,0,s)=\phi^s(x) &,x\in\partial\Omega\end{cases}\]
using the heat semigroup.

We define the by \(\eta\) scaled approximation function with ellipticized homogeneity
\[\rho_\eta(x,s):=w(x,\eta^2s^2,s),\]
and the difference function
\[\theta_\eta(x,s):=\phi^s(x)-\rho_\eta(x,s).\]






\subsection{The different parts of the derivatives of \(\theta\)}

We will have to take the partial derivative of \(\theta_\eta\) in the transversal \(t\)-direction. Thereby, we see that
\[\partial_s \theta_\eta(x,s)=\partial_s \phi^s - \partial_s w(x,\eta^2s^2,s)=\partial_s\phi^s-\partial_t w(x,t,s)|_{t=\eta^2 s^2}-\partial_s w(x,t,s)|_{t=\eta^2 s^2}.\]

We can calculate the second and third term more explicitly. For the first of them we get
\begin{align*}
    \partial_t w(x,t,s)|_{t=\eta^2 s^2}=2\eta^2 s L^s w(x,\eta^2 s^2,s).
\end{align*}

For the second one we need to work a bit more. To start with we can observe that
\begin{align*}
    \partial_s\partial_t w(x,t,s)&=\partial_s \Div(\AP(x,s)\nabla w(x,t,s))
    \\
    &=\Div(\partial_s \AP(x,s)\nabla w(x,t,s))+L^s\partial_sw(x,t,s).
\end{align*}
We can now set \(v_1(x,t)\) as the solution to
\[\begin{cases} \partial_t v_1(x,t)=L^s v_1(x,t) + \Div(\partial_s \AP(x,s)\nabla w(x,t,s)) &\textrm{for }(x,t)\in\Omega, \\ v_1(x,0)=0 &\textrm{for }(x,0)\in\partial\Omega,\end{cases}\]
and \(v_2(x,t)\) as the solution to 
\[\begin{cases} \partial_t v_2(x,t)=L^s v_2(x,t) &\textrm{for }(x,t)\in\Omega, \\ v_2(x,0)=\partial_s\phi^s(x) &\textrm{for }(x,0)\in\partial\Omega.\end{cases}\]
Since \(\partial_s w(x,0,s)=\partial_s\phi^s\) we note that \(\partial_s w\) and \(v_1+v_2\) satisfy the same linear PDE with same boundary data and hence must be equal. Next, we can give explicit representations for \(v_1\) by applying Duhamel's principle and for \(v_2\) by the heat semigroup. These are
\[v_1(x,t,s)=\int_0^t e^{-(t-\tau)L^s}\Div(\partial_s A(x,s)\nabla w(x,\tau,s))d\tau,\]
and
\[v_2(x,t,s)=e^{-tL^s}\partial_s\phi^s(x).\]
Together we get for the derivative of \(\theta\) in t-direction
\begin{align*}
    \partial_s \theta(x,s)&=\partial_s\phi^s-2\eta^2 s L^s w(x,\eta^2 s^2,s)-e^{-\eta^2s^2L^s}\partial_s\phi^s(x)
    \\
    &\qquad-\int_0^{\eta^2s^2} e^{-(\eta^2s^2-\tau)L^s}\Div(\partial_s A(x,s)\nabla w(x,\tau,s))d\tau
    \\
    &=\partial_s\phi^s-2\eta^2 s L^s w(x,\eta^2 s^2,s)-e^{-\eta^2s^2L^s}\partial_s\phi^s(x)
    \\
    &\qquad-\int_0^{s} 2\eta^2\tau e^{-\eta^2(s^2-\tau^2)L^s}\Div(\partial_s A(x,s)\nabla w(x,\eta^2\tau^2,s))d\tau
    \\
    &\eqcolon \partial_s\phi^s(x)-w_t(x,s)-w_s^{(1)}(x,s)-w_s^{(2)}(x,s).
\end{align*}




==> KatoPrelims.tex <==
\section{Consequences of the Kato conjecture}


The following result can be found as Theorem 4.77 in \cite{hofmann_lp_2022}. Note that we define \(\dot W^{1,p}(\mathbb{R}^n)\) as the closure of \(C_0^\infty(\mathbb{R}^n)\) under the seminorm given by \(\Vert f\Vert_{\dot W^{1,p}}:=\Vert \nabla f\Vert_{L^p(\mathbb{R}^n)}\).
\begin{prop}\label{prop:KatoConjecture}
    For a function \(f\in \dot W^{1,p}(\mathbb{R}^n)\) we have
    \[\Vert L^{1/2} f\Vert_{L^p(\mathbb{R}^n)}\leq C(n,\lambda_0,\Lambda_0)\Vert \nabla f\Vert_{L^p(\mathbb{R}^n)}\]
    for all \(1<p<\infty\). Furthermore, there exists \(\varepsilon_1>0\) such that if \(1<p<2+\varepsilon_1\) then
    \[\Vert \nabla f\Vert_{L^p(\mathbb{R}^n)}\leq C(n,\lambda_0,\Lambda_0)\Vert L^{1/2} f\Vert_{L^p(\mathbb{R}^n)}.\]
\end{prop}

A direct consequence is the following corollary 
\begin{cor}\label{cor:NablaL^-1/2Bounded}
    For a function \(f\in L^2(\mathbb{R}^n)\) we have
    \[\Vert \nabla L^{-1/2} f\Vert_{L^2(\mathbb{R}^n)}\approx\Vert f\Vert_{L^2(\mathbb{R}^n)}\]
    and if f is a vector valued function
    \[\Vert L^{-1/2} \Div(f)\Vert_{L^2(\mathbb{R}^n)}\approx\Vert f\Vert_{L^2(\mathbb{R}^n)}.\]
\end{cor}

==> ReductionOfLocalSqFctBound.tex <==
\section{Reduction of the local square function bound on a "good set"}

According to \cite{dindos_bmo_2017} it is enough to show the local square function bound
\begin{align}\sup_{\Delta\subset\partial\Omega}\sigma(\Delta)^{-1}\int_{T(\Delta)}\vert\nabla u\vert^2\delta dX\lesssim \Vert f\Vert^2_{L^\infty(\partial\Omega)}\label{SquarefctBound}\end{align}
to get \(\omega\in A_\infty(d\sigma)\). Combining this with the idea from Lemma 2.14 in \cite{auscher_extrapolation_2001} we only need to show (\ref{eq:SqFctonSawtooth}) to obtain \(\omega\in A_\infty(d\sigma)\). 

\begin{thm}\label{thm:ReductionOfSquareFunctionBoundToSquareFunctionBoundOnSawtoothRegion}
Let \(u\in W^{1,2}(\Omega)\) be a solution, \(\Delta\subset \partial\Omega\) a boundary cube, \(0<\eta<1\) and \(\beta<\infty\) and \(\alpha(\eta)>1\) sufficiently large. If for any subcube \(Q\subset\Delta\) there exists a open subset \(F\subset Q\) with \(|F|\geq \eta |Q|\) and
\begin{align}\int_{\tilde{\Omega}_\alpha(F)}|\nabla u|^2t dxdt\leq \beta|Q|\label{eq:SqFctonSawtooth}\end{align}
then
\[\int_{T(\Delta)}|\nabla u|^2t dxdt\leq C(\eta)\beta|Q|\]
\end{thm}

For completeness we include a proof.

\begin{proof}
Let \(\varepsilon>0\). Define
\[M(\varepsilon):=\sup_{Q\subset\Delta}\frac{1}{|Q_i|}\int_{T(Q)\cap\{t>\varepsilon\}}|\nabla u|^2tdxdt.\]
Since \(\nabla u\in L^2(\Omega)\) the value of \(M(\varepsilon)\) is bounded from above and hence exists.
Now take the open set \(F\subset \Delta\) with the given properties, and define the "left-over set" \(L_F:=T(\Delta)\setminus \tilde{\Omega}_\alpha(F)\subset\Omega\). Since \(F\) is open there is a Whitney decomposition \(F=\bigcup_{i\in \mathbb{N}} Q_i\). Due to the construction of the saw-tooth region \(\tilde{\Omega}_\alpha(F)\) we have for sufficiently large \(\alpha\) that \(L_F\subset \bigcup_{i\in \mathbb{N}} T(Q_i)\). Hence we we get
\begin{align*}
    \int_{T(\Delta)\cap\{t>\varepsilon\}}|\nabla u|^2tdxdt& =\int_{\tilde{\Omega}(F)\cap\{t>\varepsilon\}}|\nabla u|^2tdxdt+\int_{L_F\cap\{t>\varepsilon\}}|\nabla u|^2tdxdt
    \\
    &\leq \int_{\tilde{\Omega}(F)}|\nabla u|^2tdxdt + \sum_{i\in \mathbb{N}}\int_{T(Q_i)\cap\{t>\varepsilon\}}|\nabla u|^2tdxdt
    \\
    &\leq \beta|\Delta| + \sum_{i\in \mathbb{N}}|Q_i|M(\varepsilon)
    \\
    &\leq \beta |\Delta| + M(\varepsilon)|\Delta\setminus F|
    \\
    &\leq \beta |\Delta| + (1-\eta)M(\varepsilon)|\Delta|.
\end{align*}
We can devide both sides by \(|\Delta|\) and observe that the inequality
\[\frac{1}{|Q|}\int_{T(Q)\cap\{t>\varepsilon\}}|\nabla u|^2tdxdt\leq \beta+(1-\eta)M(\varepsilon)\]
holds true for all subcubes \(Q\subset \Delta\). Hence we have
\[M(\varepsilon)\leq \beta+(1-\eta)M(\varepsilon),\]
which implies the statement we wanted to show via letting \(\varepsilon\to 0\).


\end{proof}

==> TheGoodSetF.tex <==
\section{The good set F and local estimates on F}

We would like to bound the family \(|\nabla \phi^t|\) uniformly in \(t\).
If we have a Hodge decomposition in \(n=1\) on \(\Delta=(a, a+l(\Delta))\), we note that
\[\partial_x(c(x,t))=L^t\phi^t=\partial_x(\AP(x,t)\partial_x\phi^t),\]
and we can compute the solution \(\phi^t\) by integration as
\[\phi^t(x)=\int_{a}^x c(x,t)dx - \int_{a}^{l(\Delta)} c(x,t)dx. \]
Thus, we have a uniform pointwise bound on \(\nabla \phi^t\):


\begin{lemma}\label{lemma:UniformBoundOnM[nablaphi^s]}
If \(n=1\), we have
\[M[|\partial_x\phi^s|](x)\leq C(\Lambda_0)l(\Delta),\]
and 
\[\Vert M[\nabla\phi^s]\Vert_{L^2}\leq C(\Lambda_0)l(\Delta).\]
As a consequence, we also observe that for small \(\gamma>0\) there exists a large \(\kappa_0>0\) and \(F\subset 3\Delta\) such that
\[M[|\partial_x\phi^s| ](x)\leq M[|\partial_x\phi^s|^2]^{1/2}(x)\leq C(\lambda_0,\Lambda_0)\kappa_0\qquad \textrm{for all }x\in F, \textrm{ and }s>0,\]
where \(|3\Delta\setminus F|\leq \gamma |\Delta|\).
\end{lemma}














This lemma leads to the following lemma which will be used in the proof of \refthm{thm:MainTheorem}.

\begin{lemma}\label{lemma:thetaPointwiseBoundOnGoodSetF}
Assume \ref{condition:L^1Carlesontypecond}. Then for small \(\gamma>0\) there exists a large \(\kappa_0>0\) and \(F\subset 3\Delta\) such that
\[\theta_\eta(x,s)\leq C(n,\lambda_0,\Lambda_0)\kappa_0\eta s\qquad \textrm{for all }x\in F, s>0\]
where \(|3\Delta\setminus F|\leq \gamma |\Delta|\).
\end{lemma}

\begin{proof}
We take F from \reflemma{lemma:UniformBoundOnM[nablaphi^s]}. By
\refcor{cor:PointwiseBoundsofw_tAndrhoByM(nablaphi^s)} we have \(\partial_t w(y,(\eta t)^2,s)\leq C(n,\lambda_0,\Lambda_0) \eta M[\nabla\phi^s](y)\) for all \(y\in \mathbb{R}^n\). Hence we get from \reflemma{lemma:UniformBoundOnM[nablaphi^s]} for \(x\in F\)
\[\theta_\eta(x,s)=\int_0^s \partial_t w(x,(\eta t)^2,s)dt\lesssim \int_0^s \eta\kappa_0 dt\leq \kappa_0\eta s.\]
\end{proof}

The next lemma is an extension of \reflemma{lemma:thetaPointwiseBoundOnGoodSetF}.

\begin{lemma}\label{lemma:thetaPointwiseBoundOnOmega(F)}
Assume \ref{condition:L^1Carlesontypecond}. Then for small \(\gamma>0\) there exists a large \(\kappa_0>0\) such that
\[\theta_\eta(x,s)\leq C(n,\lambda_0,\Lambda_0)\kappa_0\eta s\qquad \textrm{for all }(x,s)\in \tilde{\Omega}(F)\]
where \(F\subset 3\Delta\) with \(|3\Delta\setminus F|\leq \gamma |\Delta|\).
\end{lemma}

\begin{proof}
    Analogously to Lemma 8 in \cite{hofmann_dirichlet_2022}.
\end{proof}


In the following lemma we use a ball just in spatial direction, i.e.
\[B_x(x,t):=\{(y,s); |y-x|<\frac{t}{2}\big\},\]
and adjust \refprop{Proposition12} to our case. 
 Instead of showing an in \(s\) uniform bound of the nontangential maximal functions we just need the following.

\begin{lemma}\label{lemma:UnifromBoundOnrholocally}
Let \(\alpha>0,\eta>0\) and \(F\) like in \reflemma{lemma:UniformBoundOnM[nablaphi^s]}. For \(x\in F\) we have
\[\fint_{B_x(x, {\eta\alpha} s)}|\nabla\rho_\eta(y,s)|^2 dy \lesssim_{\alpha,\eta} \kappa_0 \qquad\textrm{for all }(x,s)\in \tilde{\Omega}_{\eta\alpha}(F).\]
\end{lemma}

\begin{proof}
Fix \(0<\EPS< \frac{1}{100}\) small and let \(\psi\in C^\infty\) be a smooth cut-off function with \(\mathrm{supp}(\psi)\subset (1+\EPS)B_x(x,{\eta\alpha} s)\) and \(\psi\equiv 1\) on \(B(x,{\eta\alpha} s)\), while \(|\partial_t\psi| + |\nabla\psi|\lesssim \frac{1}{{\EPS\eta\alpha} s}\). We choose \(m:=\fint_{B_x(x, 2\eta\alpha s)}\phi^s(x) dx=(\phi^s(\cdot))_{B_x(x, 2\eta\alpha s)}\) and note that \(\nabla m=0\). Then we get
\begin{align*}
    \fint_{B_x(x,{\eta\alpha} s)}|\nabla\rho_\eta|^2 dy&\leq \fint_{(1+\EPS)B_x(x,{\eta\alpha} s)}A\nabla\rho_\eta\cdot \nabla\rho_\eta \psi^2 dy
    \\
    &= \fint_{(1+\EPS)B_x(x,{\eta\alpha} s)}A\nabla\rho_\eta\cdot \nabla(\rho_\eta-m) \psi^2 dy
    \\
    &=\fint_{(1+\EPS)B_x(x,{\eta\alpha} s)}A\nabla\rho_\eta\cdot \nabla((\rho_\eta-m) \psi^2) dy
    \\
    &\qquad + \fint_{(1+\EPS)B_x(x,{\eta\alpha} s)}A\nabla\rho_\eta\cdot (\rho_\eta-m) \psi\nabla\psi dy \eqcolon I+J.
\end{align*}
Since \(s L^s \rho_\eta(x,s)=w_t(x,s)\) we have by \refcor{cor:PointwiseBoundsofw_tAndrhoByM(nablaphi^s)}
\[I=\fint_{(1+\EPS)B_x(x,\eta\alpha s)}w_t(y,s) \frac{(\rho_\eta(y,s)-m)\psi^2}{\eta\alpha s} dy\lesssim M[\nabla\phi^s](P)^2\]
for every \((P,s)\in \Gamma_{\eta\alpha}(x)\). Choosing \(P\in F\) leads with \reflemma{lemma:UniformBoundOnM[nablaphi^s]} to \(I\lesssim \kappa_0^2\).

\medskip

For \(J\) we can calculate for \(0<\sigma<1\)
\begin{align*}
J&\lesssim \Big(\fint_{(1+\EPS)B_x(x,\eta\alpha s)}|\nabla\rho_\eta|^2\psi^2 dy\Big)^{1/2}\Big(\fint_{(1+\EPS)B_x(x,\alpha\eta s)}\frac{|\rho_\eta-m|^2}{s^2} dy\Big)^{1/2}
\\
&\lesssim \sigma \fint_{(1+\EPS)B_x(x,\alpha\eta s)}|\nabla\rho_\eta|^2\psi^2 dy+ M[\nabla\phi^s](P)^2
\\
&\leq \sigma \fint_{(1+\EPS)B_x(x,\alpha\eta s)}|\nabla\rho_\eta|^2\psi^2 dy+ \kappa_0^2.
\end{align*}
Hiding the first term on the left side yields
\[\fint_{B_x(x,\alpha\eta s)}|\nabla\rho_\eta|^2 dy\lesssim \kappa_0^2.\]
\end{proof}


==> introduction.tex <==
\section{Introduction}

We are interested in the solvability of the \(L^p\) Dirichlet boundary value problem for linear elliptic PDEs, which is the solvability of 
\[\begin{cases} \mathcal{L}u=\Div(A\nabla u)=0 &\textrm{in }\Omega, \\ u=f &\textrm{on }\partial\Omega,\end{cases}\]
where \(f\in L^p(\partial\Omega)\). This problem has been studied extensively in the last decades going back to an observation of Dahlberg in \cite{dahlberg_estimates_1977} where he proved that the \(L^2\) Dirichlet problem is solvable for the Laplacian on a Lipschitz domain. Since then much progress has been made and two main types of conditions appeared as sufficient criteria for \(L^p\) Dirichlet solvability for some \(1<p<\infty\) or equivalently for \(\omega\in A_\infty(\sigma)\), which means that the elliptic measure lies in a Muckenhoupt class of the surface measure on the boundary. These two conditions are the Carleson condition whose operators are also called DKP-operators and the t-independence condition.
\\

In our present work let \(\Omega:=\mathbb{R}^{n+1}_+:=\mathbb{R}^n\times [0,\infty)\) be the upper half space and \(\mathcal{L}:=\Div(A\nabla\cdot)\) an uniformly elliptic operator, i.e. there exists \(\lambda_0>0\)
\begin{align}
    \lambda_0 |\xi|^2\leq \xi^T A(x,t) \xi \leq \lambda_0^{-1}|\xi|^2 \qquad \textrm{ for all }\xi\in \mathbb{R}^{n+1},\label{eq:DefinitionOfUniformElliptic}
\end{align}
and a.e. \((x,t)=(x_1,...,x_n,t)\in \mathbb{R}^{n+1}_+\). We do not necessarily require symmetry of the matrix \(A\) in the following, though we would like to mention that implicit in our definition of ellipticity we can find boundedness of \(A\).

\medskip

In this setting we say an elliptic operator \(\mathcal{L}\) satisfies the t-independence condition if \(A(x,t)=A(x)\) for all \(x\in \mathbb{R}^n\) and \(t>0\), i.e. the matrix A is independent of the direction perpendicular to the boundary. First, \cite{jerison_kenig_1981} showed that if \(A\) is symmetric and t-independent, we have \(\omega\in A_\infty(\sigma)\) via a "Rellich" identity. It took until the Kato conjecture was resolved in \cite{Auscher_Kato} after being open for 50 years, before the authors of \cite{hofmann_regularity_2014} could extend this result to matrices that are not necessarily symmetric and have just bounded and measurable coefficients. Later, this work got streamlined in \cite{hofmann_dirichlet_2022} where the authors also extend the result to the case of matrices whose antisymmetric part might be unbounded and instead has a uniformly bounded BMO norm of its antisymmetric part. 

\medskip

In our work we go back to the case of bounded matrices with measurable coefficients which might be non symmetric. We introduce a mixed \(L^1-L^\infty\) type Carleson condition on \(\partial_t A(x,t)\), i.e.
\begin{align}\int_0^\infty\Vert\partial_t A(\cdot,t)\Vert_{L^\infty(\mathbb{R}^n)} ds\leq C<\infty.\label{condition:L^1Carlesontypecond}\end{align}
This condition essentially takes the \(L^\infty\) norm of \(\partial_t A(x,t)\) in x-direction first, before imposing some quantified form of decay close to 0 and to infinity as \(L^1\) norm. This result extends the previous t-independence condition from \cite{hofmann_regularity_2014}, since the matrices here are allowed to depend on the perpendicular direction t as long as their behaviour in this direction is not too bad. The main theorem of this work is the following.

\begin{thm}\label{thm:MainTheorem}
Let \(L:=\Div(A\nabla\cdot)\) be an elliptic operator satisfying \ref{eq:DefinitionOfUniformElliptic} on \(\Omega=\mathbb{R}^{n+1}\). If condition \ref{condition:L^1Carlesontypecond} is satisfied and \(\frac{|\partial_t A|}{t}\leq C<\infty\) then \(\omega\in A_\infty(d\sigma)\), i.e. the \(L^p\) Dirichlet boundary value problem for \(L\) is solvable for some \(1<p<\infty\).
\end{thm}

All of the following chapter with the exception of the last one are preliminary calculations and definitions before the last section shows the proof of the main theorem. Our proof idea is inspired by the proof in \cite{hofmann_dirichlet_2022} and a sketch of the technical proof is given where we also point out the major differences that require more delicate handling of the operators involving the heat semigroup.
